HARP: A Large-Scale Higher-Order Ambisonic Room Impulse Response Dataset

This contribution introduces a dataset of 7th-order Ambisonic Room Impulse Responses (HOA-RIRs), created using the Image Source Method. By employing higher-order Ambisonics, our dataset enables precise spatial audio reproduction, a critical requirement for realistic immersive audio applications. Leveraging the virtual simulation, we present a unique microphone configuration, based on the superposition principle, designed to optimize sound field coverage while addressing the limitations of traditional microphone arrays. The presented 64-microphone configuration allows us to capture RIRs directly in the Spherical Harmonics domain. The dataset features a wide range of room configurations, encompassing variations in room geometry, acoustic absorption materials, and source-receiver distances. A detailed description of the simulation setup is provided alongside for an accurate reproduction. The dataset serves as a vital resource for researchers working on spatial audio, particularly in applications involving machine learning to improve room acoustics modeling and sound field synthesis. It further provides a very high level of spatial resolution and realism crucial for tasks such as source localization, reverberation prediction, and immersive sound reproduction.

==> notes.tex <==


\subsection{Energy Decay Curves (EDC)}
Figure \ref{fig:EDC} displays Energy Decay Curves (EDCs) for five randomly selected samples. The EDC plots, measured in decibels, show the energy decay patterns over time, demonstrating the diversity in room configurations within the dataset. Each EDC reflects different reverberation characteristics, including rapid decay in smaller, highly absorptive rooms and slower decay in larger, reflective spaces.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.1\columnwidth]{EDCs.png}
    \caption{Energy Decay Curve calculated with $0^{th}$-order microphone of 5 random RIR samples.}
    \label{fig:EDC}
\end{figure}}
